Plug-and-Play Diffusion Distillation

Diffusion models have shown tremendous results in image generation. However, due to the iterative nature of the diffusion process and its reliance on classifier-free guidance, inference times are slow. In this paper, we propose a new distillation approach for guided diffusion models in which an external lightweight guide model is trained while the original text-to-image model remains frozen. We show that our method reduces the inference computation of classifier-free guided latent-space diffusion models by almost half, and only requires 1\% trainable parameters of the base model. Furthermore, once trained, our guide model can be applied to various fine-tuned, domain-specific versions of the base diffusion model without the need for additional training: this "plug-and-play" functionality drastically improves inference computation while maintaining the visual fidelity of generated images. Empirically, we show that our approach is able to produce visually appealing results and achieve a comparable FID score to the teacher with as few as 8 to 16 steps.

==> rebuttal.tex <==
% \documentclass[10pt,twocolumn,letterpaper]{article}
% \usepackage[rebuttal]{cvpr}

% % Include other packages here, before hyperref.
% \usepackage{graphicx}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{booktabs}

% \usepackage{wrapfig}

% % Import additional packages in the preamble file, before hyperref
% \input{preamble}

% % If you comment hyperref and then uncomment it, you should delete
% % egpaper.aux before re-running latex.  (Or just hit 'q' on the first latex
% % run, let it finish, and you should be clear).
% \definecolor{cvprblue}{rgb}{0.21,0.49,0.74}
% \usepackage[pagebackref,breaklinks,colorlinks,citecolor=cvprblue]{hyperref}

% % Support for easy cross-referencing
% \usepackage[capitalize]{cleveref}
% \crefname{section}{Sec.}{Secs.}
% \Crefname{section}{Section}{Sections}
% \Crefname{table}{Table}{Tables}
% \crefname{table}{Tab.}{Tabs.}

% % If you wish to avoid re-using figure, table, and equation numbers from
% % the main paper, please uncomment the following and change the numbers
% % appropriately.
% %\setcounter{figure}{2}
% %\setcounter{table}{1}
% %\setcounter{equation}{2}

% % If you wish to avoid re-using reference numbers from the main paper,
% % please uncomment the following and change the counter for `enumiv' to
% % the number of references you have in the main paper (here, 6).
% %\let\oldthebibliography=\thebibliography
% %\let\oldendthebibliography=\endthebibliography
% %\renewenvironment{thebibliography}[1]{%
% %     \oldthebibliography{#1}%
% %     \setcounter{enumiv}{6}%
% %}{\oldendthebibliography}


% %%%%%%%%% PAPER ID  - PLEASE UPDATE
% \def\paperID{6962} % *** Enter the Paper ID here
% \def\confName{CVPR}
% \def\confYear{2024}

% \begin{document}

% %%%%%%%%% TITLE - PLEASE UPDATE
% \title{Author Response - Plug and Play Diffusion Distillation}  % **** Enter the paper title here

% \maketitle
% \thispagestyle{empty}
% \appendix
% \input{sec/rebuttal}

% % We thank the reviewers for the time and expertise 
% % they have invested in these reviews. We appreciate positive comments about the paper like {\color{red}Siavash: let's mention a couple of good comments}
% % Furthermore, the insightful comments we received point us towards several directions in which this work can be extended in the future. We focus on answering to the posed questions by the reviewers and provide feedback related to improvements suggestions.
% % Thanks for the reviewers' response. 
% % % We apologize for some of the 


% % \underline{Combined Response}

% % \noindent{\textbf{Fig 5 \& Fig 8. Display Each column with the same text prompts (YXGL, g4Qk, tesf)}}
% % % Our initial goal for Fig 5 and 8 is supposed to be generally showing the overall ability of each model being albe to show high quality images, yet we acknowledged that it may be misleading if  each column in Fig 5 are displayed with different textprompts.


% % We would like to adopt the reviewers’ suggestions and align the text prompt for each column. To save space, we'll present one column\footnote{\label{explain1} We changed it into a row in the rebuttal document for better display} for display:

% % \begin{figure}[h]
% % \centering
% %     \includegraphics[width=1\linewidth]{figures/rebuttal-same-textprompts.png}
% %     \centering
% %     % \caption{TBA}
% %     \label{fig:rebuttal-same-txtprompts}
% % \end{figure}

% % In the camera-ready version, the layout would be something that looks like Figure 9 \footnote{\label{explain2} Fig 9 is in Appendix/Supplementary Material}, but we will perform a variety of text prompts.
% % % instead of focusing on generating different styles.
% % The same means will be applied to Fig 8.\\

% % \noindent{\textbf{Original guide model is full guide model (YXGL, tesf)}}
% % We apologize for any confusion. All instances of the original guide model will be amended to the full guide model in the camera-ready version.\\

% % \noindent{\textbf{Detailed Tiny model architecture (tesf, g4Qk)}}
% % $\gamma$ is the guidance vector, which is a vector of guidance number $g$. On the other hand, timestep embedding and text embedding will also pass through zero convolution layers, denoted $Z(\cdot, \cdot)$. 
% % % Specifically, $Z(\cdot, \cdot)$ is a convolution layer with both weight and bias initialized to zeros.
% % Finally, these elements will be added together and pass through the zero convolutions in the decoding layer to get the corresponding output:
% % \begin{equation}
% % y = Z\left(\gamma + Z(c_{timestep}; \Theta_{z1}) + Z(c_{text}; \Theta_{z2}); \Theta_{z3}\right)
% % \end{equation}
% % where $y$ is the output of the guide model. Zero convolution architecture intends to make sure that it will not be "injecting garbage" into the base model in the early stage of the training.\\
 
% % \textbf{FID scores of our methods are relatively high when guidance is small (g=2, 4, 6) in Table 2 (g4Qk, YXGL)}
% % Table 2 of course conveys various information, but among them, we key point wanted to convey is that the training of the model is stable given a certain level of guidance. Please note that the training of the model was recorded as FID 23.97 for the tiny model fixed guidance 8. When the guidance is small, the injection noise is small, and can be close to the guidance = 0 where it’s the same as not having CFG at all. And we know that without CFG image quality is low.
% % We would add this part of the discussion in the original context too.\\
% % % \section{Line-by-line Individual Response}

% % \begin{figure}[h]
% % \centering
% %     \includegraphics[width=1\linewidth]{figures/rebuttal-baseline-comp.png}
% %     \centering
% %     \caption{TBA}
% %     \label{fig:rebuttal-baseline-comp}
% % \end{figure}
% % % \begin{enumerate}
% % %     \item \textbf{FID scores of full \& tiny goes up from 50 steps to 16 steps in g=6}
% % %         \item This table of course conveys various information, but among them, we wanted to say that the training of the model is stable given a certain level of guidance. Please note that the training of the model was recorded as FID 23.97 for the tiny model fixed guidance 8. When the guidance are small, the injection noise are small, and can be close to the guidance = 0 where it’s exactly the same as not having CFG at all. And we know that without CFG image quality is low.
% % %     \end{enumerate}
% % \section{Reviewer YXGL}
% % \textbf{[{\relax}...]The paper should include baselines for other sampling step distillation methods as a comparison for both quantitative and qualitative evaluation.}
% % Most existing distillation methods focus on sampling steps distillation, under the scenario of unguided diffusion models, which may it hard to compare with them. That’s why we didn’t include them at the first place. This\footnote{\label{Ondist}https://arxiv.org/pdf/2210.03142.pdf} is a paper that includes CFG distillation. As such, we could add this method to our paper as one of our baselines. We would also like to add this \footnote{\label{Dpm++} https://arxiv.org/pdf/2211.01095.pdf} for the baseline comparisons. \fref{fig:rebuttal-baseline-comp} is the qualitative comparison of the methods. The FIDs of these models are \tref{tab:baselines-compareisons}. Also, we would like to emphasize that our method fixes the base model, and the training parameters \& computational cost is way lower then the paper, On Distillation Guided Diffusion Models, while achieving similar FID scores when guidance=8. teacher is the upper bound of its students’ performance and it’s better to compare our method with DPM++ when we’re also using DPM++ as our scheduler.\\
% % % \item \textbf{Figure 5 is confusing to me. Do the images in one column correspond to the same prompt/starting latent? It is hard for me to judge these images in the way they are presented, am I supposed to compare the 3 teddy bears to the astronaut? And why are the same subjects (chocolate cake, cats) not in the same column?}
% % % \begin{enumerate}
% % %     \item reply in combined response, section\textit{ Remaking Fig 5 \& Fig 8. Display Each column with the same textprompts}
% % % \end{enumerate}
% % % \item \textbf{Also, is the original guide model the same as the full guide model? If so, why do they have different names in the same figure?}
% % % \begin{enumerate}
% % %     \item replied in combined response, section \textit{Original guide model is the Full guide model}
% % % \end{enumerate}
% % \textbf{ Why is the tiny model shown with 50 and 16 steps but the full one with 8 and 16? }
% % The reason is because of the light-weight nature of the tiny model made the performance of 8 steps not as good as the full model, and displaying it’s evaluation results may be meaningless. \\
% % \textbf{[{\relax}...]it might be beneficial to include the standard CFG update with x steps in  Figure [{\relax}...]}
% % Thanks for reviewers suggestion. We would update \textit{"CFG"} with \textit{"CFG 50 steps"} in Figure 6 accordingly.\\
% % \textbf{Include a user study that shows that users do not (strongly) favor the images with 50 CFG steps over student \& teacher. Fig 6 looks artificial.}
% % One of the characteristics observed from the injection-based conditioned model (e.g. controlnet) is that they are more saturated and have higher contrast.  Some may think that it looks less realistics, yet others may think that it’s more visually pleasing. This characteristics also persists in our model. But don’t worry, saturation can be alleviate by tuning the guidance number lower. We acknowledge that one’s taste over pictures may be more subjective, so we adopt the reviewer’s suggestion to conduct a user study. Specifically, …\\
% % \section{Reviewer g4Qk}
% % % \begin{enumerate}
% %     % \item \textbf{The paper is a bit confusing. For example, it fails to draw a stronger connection to ControlNets, including the crucial detail how the feature maps are "injected" to the main path. I'm assuming this is just an addition like in ControlNet's "zero convolution" paths, but this definitely should be in the text and diagrams to have a self-contained story. Fig 4 is way too abstract}
% %     % \begin{enumerate}
% %     %     \item replied in combined response, section \textit{Detailed Tiny model architechture}
% %     % \end{enumerate}
% % \textbf{ [{\relax}...]L337-L341 [{\relax}...] "In practice" when in fact you tried to say that "without your invention" [{\relax}...]}
% % We would modify this context accordingly. We would also double check if there are other similar context-setting that would be misleading to our readers in our camera-ready version.\\
% % \textbf{L320 remarks \& discussions}
% %     % \begin{enumerate}
% %         % \item
% %         Since the tiny guide model only has limited parameter capacities to learn, it may be hard for it to mimic the teacher’s output under a variety of guidance values. Thus, we also tried to train a tiny model with a fixed guidance. 
% %         % It would significantly reduce the FID scores from 36.22 to 23.97. 
% %         This trick is also used in other papers\footref{Ondist}. \\
% %     % \end{enumerate}
% % \textbf{For DDIM, 16 steps is worse than 8 steps in Table 2?
% % % Also, I don't think these numerical results unambiguously support your story. For example, with g=2,4,6 FID is pretty bad for 50 steps, etc. I'm not satisfied with how the numbers and story combine.
% % }
% % We apologize to our typo. The numerical numbers of 16 steps and 8 steps are reversed. We will double-check and revise the table in the camera-ready version.
% % % \item \textbf{Figures 5 \& 8 [{\relax}...] don't even have fixed prompts per column [{\relax}...] }
% % % \begin{enumerate}
% % %     \item reply in combined response, section \textit{Remaking Fig 5 \& Fig 8. Display Each column with the same textprompts}
% % % \end{enumerate}
% % % \end{enumerate}
% % \section{Reviewer tesf}
% % % \begin{enumerate}
% % %     \item \textbf{I do not understand what the "tiny" guide model architecture is [{\relax}...]}
% % %     \begin{enumerate}
% % %         \item replied in combined response, section\textit{ Detailed Tiny model architechture}
% % %     \end{enumerate}
% % % \item \textbf{[{\relax}...] I think a much stronger point would be made by using the same text prompts in each column [{\relax}...]}
% % % \begin{enumerate}
% % %     \item reply in combined response, section\textit{ Remaking Fig 5 \& Fig 8. Display Each column with the same textprompts}
% % % \end{enumerate}
% % \textbf{How does our methods work on pixel-based diffusion models (e.g., Imagen)}
% % Thanks for the reviewer's input. We would definitely like to add this in our future study.


% % % \end{enumerate}
% % % \end{enumerate}


% % % [DONE] In overleaf let’s add rebuttal document so we can start working on it
% % % Bring baselines (FID) from other papers + visual comparison (e.g DDIM++)
% % % combine fig 5 & 6 in the future. Just one column is enough
% % % repick figure 5 by inference the model
% % % also can say we have images with they same prompts
% % % point to supplemental material figure 9 as well

% % % user study? Generate 50 steps DDIM vs our method and do user study (A/B testing) Goal: 500 images 
% % % Tiffany to provide 500 prompts

% % % detailed explanation on tiny model arch + fig (Tiffany)

% % \input{sec/tab-and-figs/tab-new-comparison}

% % % \section{Integrated Response}
% % % \subsection{Display of Fig. 5}
% % % \subsection{Detailed explanation of tiny model arch and fig}
% % % \section{Reviewer YXGL}

% % % \subsection{Regarding display of Fig. 5}
% % % \section{Reviewer g4Qk}
% % % % \begin{itemize}

% % % \noindent{\bf The paper is a bit confusing. For example, it fails to draw a stronger connection to ControlNets, including the crucial detail how the feature maps are "injected" to the main path. I'm assuming this is just an addition like in ControlNet's "zero convolution" paths, but this definitely should be in the text and diagrams to have a self-contained story. Fig 4 is way too abstract.}

% % % \noindent{\bf  The text has some causality issues. For example, on lines L337-L341 it was confusing to read "In practice" when in fact you tried to say that "without your invention" this and that. Practical concerns always apply, you see. Please be more careful with these sort of context-setting statements.}

% % % \noindent{\bf  Some interesting remarks, like L320 (fixed guidance in tiny model), are just thrown out there, while these are exactly the things that deserve discussion.
% % % }
% % % \noindent{\bf  Table 2 is confusing. For DDIM, 16b steps is worse than 8 steps?! This must be an error. Also, I don't think these numerical results unambiguously support your story. For example, with g=2,4,6 FID is pretty bad for 50 steps, etc. I'm not satisfied with how the numbers and story combine.}

% % %     \begin{itemize}
% % %         \item please be satisfied...
% % %     \end{itemize}
    
% % % \noindent{\bf Figures 5 & 8 are confusing. A bunch of hand-picked images, that don't even have fixed prompts per column? What am I supposed to see in here? This kind of visuals fail to tell me anything, except maybe that it's not broken/adversarial attack against metrics.}
% % % % \end{itemize}

% % % \section{Reviewer tesf}



% % % [DONE] In overleaf let’s add rebuttal document so we can start working on it
% % % Bring baselines (FID) from other papers + visual comparison (e.g DDIM++)
% % % combine fig 5 & 6 in the future. Just one column is enough
% % % repick figure 5 by inference the model
% % % also can say we have images with they same prompts
% % % point to supplemental material figure 9 as well

% % % user study? Generate 50 steps DDIM vs our method and do user study (A/B testing) Goal: 500 images 
% % % Tiffany to provide 500 prompts

% % % detailed explanation on tiny model arch + fig (Tiffany)

% % % %%%%%%%%% BODY TEXT - ENTER YOUR RESPONSE BELOW
% % % % \section{Introduction}

% % % % After receiving paper reviews, authors may optionally submit a rebuttal to address the reviewers' comments, which will be limited to a {\bf one page} PDF file.
% % % % Please follow the steps and style guidelines outlined below for submitting your author response.

% % % % The author rebuttal is optional and, following similar guidelines to previous conferences, is meant to provide you with an opportunity to rebut factual errors or to supply additional information requested by the reviewers.
% % % % It is NOT intended to add new contributions (theorems, algorithms, experiments) that were absent in the original submission and NOT specifically requested by the reviewers.
% % % % You may optionally add a figure, graph, or proof to your rebuttal to better illustrate your answer to the reviewers' comments.

% % % % Per a passed 2018 PAMI-TC motion, reviewers should refrain from requesting significant additional experiments for the rebuttal or penalize for lack of additional experiments.
% % % % Authors should refrain from including new experimental results in the rebuttal, especially when not specifically requested to do so by the reviewers.
% % % % Authors may include figures with illustrations or comparison tables of results reported in the submission/supplemental material or in other papers.

% % % % Just like the original submission, the rebuttal must maintain anonymity and cannot include external links that reveal the author identity or circumvent the length restriction.
% % % % The rebuttal must comply with this template (the use of sections is not required, though it is recommended to structure the rebuttal for ease of reading).

% % % % %-------------------------------------------------------------------------

% % % % \subsection{Response length}
% % % % Author responses must be no longer than 1 page in length including any references and figures.
% % % % Overlength responses will simply not be reviewed.
% % % % This includes responses where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
% % % % Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.

% % % % %------------------------------------------------------------------------
% % % % \section{Formatting your Response}

% % % % {\bf Make sure to update the paper title and paper ID in the appropriate place in the tex file.}

% % % % All text must be in a two-column format.
% % % % The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
% % % % Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
% % % % The top margin should begin 1 inch (2.54 cm) from the top edge of the page.
% % % % The bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
% % % % for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the page.

% % % % Please number any displayed equations.
% % % % It is important for readers to be able to refer to any particular equation.

% % % % Wherever Times is specified, Times Roman may also be used.
% % % % Main text should be in 10-point Times, single-spaced.
% % % % Section headings should be in 10 or 12 point Times.
% % % % All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
% % % % Figure and table captions should be 9-point Roman type as in \cref{fig:onecol}.


% % % % List and number all bibliographical references in 9-point Times, single-spaced,
% % % % at the end of your response.
% % % % When referenced in the text, enclose the citation number in square brackets, for example~\cite{Alpher05}.
% % % % Where appropriate, include the name(s) of editors of referenced books.

% % % % \begin{figure}[t]
% % % %   \centering
% % % %   \fbox{\rule{0pt}{0.5in} \rule{0.9\linewidth}{0pt}}
% % % %   %\includegraphics[width=0.8\linewidth]{egfigure.eps}
% % % %    \caption{Example of caption.  It is set in Roman so that mathematics
% % % %    (always set in Roman: $B \sin A = A \sin B$) may be included without an
% % % %    ugly clash.}
% % % %    \label{fig:onecol}
% % % % \end{figure}

% % % % To avoid ambiguities, it is best if the numbering for equations, figures, tables, and references in the author response does not overlap with that in the main paper (the reviewer may wonder if you talk about \cref{fig:onecol} in the author response or in the paper).
% % % % See \LaTeX\ template for a workaround.

% % % % %-------------------------------------------------------------------------
% % % % \subsection{Illustrations, graphs, and photographs}

% % % % All graphics should be centered.
% % % % Please ensure that any point you wish to make is resolvable in a printed copy of the response.
% % % % Resize fonts in figures to match the font in the body text, and choose line widths which render effectively in print.
% % % % Readers (and reviewers), even of an electronic copy, may choose to print your response in order to read it.
% % % % You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

% % % % When placing figures in \LaTeX, it is almost always best to use \verb+\includegraphics+, and to specify the  figure width as a multiple of the line width as in the example below


% % % % {\small\begin{verbatim}
% % % %    \usepackage{graphicx} ...
% % % %    \includegraphics[width=0.8\linewidth]
% % % %                    {myfile.pdf}
% % % % \end{verbatim}
% % % % }


% %%%%%%%%% REFERENCES
% % {
% %     \small
% %     \bibliographystyle{ieeenat_fullname}
% %     \bibliography{main}
% % }

% \end{document}


==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/rebuttal.tex <==

\definecolor{Dark blue}{RGB}{102, 153, 204}  % Dark blue
\definecolor{Dark green}{RGB}{153, 204, 102}  % Dark green
\definecolor{Dark red}{RGB}{204, 102, 102}   % Dark red

\newcommand{\rone}{{\color{Dark blue} YXGL}}
\newcommand{\rtwo}{{\color{Dark green} g4Qk}}
\newcommand{\rthree}{{\color{Dark red} tesf}}
% \clearpage
% \appendix
% \setcounter{page}{1}
% \maketitlerebuttal

We thank all the reviewers for their valuable feedback. 
We particularly appreciate the recognition of our method as an effective approach to increase efficiency while keeping the base model untouched, which made model training easy, lightweight, and interpretable (e.g. Fig 7).
In the following, we focus on answering the questions raised by the reviewers.

%We appreciate positive comments about the paper like {\color{red}Siavash: let's mention a couple of good comments. Quote from the reviewers}
%Furthermore, the insightful comments we received point us towards several directions in which this work can be extended in the future. We focus on answering to the posed questions by the reviewers and provide feedback related to improvements suggestions.\\
% Thanks for the reviewers' response. 
% We apologize for some of the 
% \underline{Combined Response}
\noindent{\textbf{[\rone, \rtwo, \rthree] Display Each column with the same text prompts in Fig 5 \& Fig 8}:}
% Our initial goal for Fig 5 and 8 is supposed to be generally showing the overall ability of each model being albe to show high quality images, yet we acknowledged that it may be misleading if  each column in Fig 5 are displayed with different textprompts.
We will adopt the reviewers’ suggestions and align the text prompt for each column. To save space, we present one column\footnote{\label{explain1}We changed it into a row in the rebuttal document for better display}:\\
\vspace{-11mm}\\
\begin{figure}[h]
\centering
    \includegraphics[width=1\linewidth]{figures/rebuttal-fig1.pdf}
    \centering
    % \caption{TBA}
    \label{fig:rebuttal-same-txtprompts}
\end{figure}
\vspace{-8mm}\\
Note that we also added full guide model 50 steps and tiny guide model (fixed guidance) 8 steps in Fig 5. for a comprehensive comparison.
% \noindent{In the camera-ready version, the layout would be like Figure 9.}
%\footnote{\label{explain2} Fig 9 is in Appendix/Supplementary Material} 
% in the supplementary material, but we will include a variety of text prompts.
% instead of focusing on generating different styles.
% The same will be applied to Fig 8.

\noindent{\textbf{[\rone, \rthree] Original guide model is full guide model:}}
The term \textit{original guide model} will be removed in the final version. We apologize for any confusion.

\noindent{\textbf{[\rtwo, \rthree] Detailed Tiny model architecture:}}
$\gamma$ is the guidance vector, which is a vector of guidance number $g$. On the other hand, timestep embedding and text embedding will also pass through zero convolution layers, denoted $Z(\cdot, \cdot)$. 
% Specifically, $Z(\cdot, \cdot)$ is a convolution layer with both weight and bias initialized to zeros.
These elements are added together and passed through the zero convolutions in the decoding layer to get the corresponding output:
\begin{equation}
y = Z\left(\gamma + Z(c_{timestep}; \Theta_{z1}) + Z(c_{text}; \Theta_{z2}); \Theta_{z3}\right)
\end{equation}
where $y$ is the guide models' output. Zero convolution architecture ensures that undesirable noise or irrelevant features are not injected into the base model in the early stage of the training. We will provide a detailed configuration and code to ensure reproducibility after the paper is published.

% \noindent{\textbf{[\rone, \rtwo] FID scores of our methods are relatively high when guidance is small (g=2, 4, 6) in Table 2}:}
% % Table 2 of course conveys various information, but among them, the main idea we wanted to convey is that the training of the model is stable given a certain level of guidance. Please note that the training of the model was recorded as FID 23.97 for the tiny model fixed guidance 8. When the guidance is small, the injection noise is small, and can be close to the guidance = 0 where it’s the same as not using CFG at all. And we know that without CFG image quality is low.
% %We would add this part of the discussion in the original context too.
% Table 2 shows that the guide model's performance is stable given a certain level of guidance. Due to the formulation of the guidance model, when the guidance value is small, the injection noise is small (as depicted in Figure 7). Therefore, the g=0 corresponds to not using CFG at all, which is known to generate low-quality images. %This can lead to the decrease in performance as guidance decreases.
% However, when guidance is higher (g=8) our model is comparable to the teacher model.

% \underline{Line-by-line Individual Response}

\begin{figure}[h]
\centering
    \vspace{-4mm}
    \includegraphics[width=1\linewidth]{figures/rebuttal-baseline-comp.pdf}
    \centering
    \vspace{-2em}
    \caption{qualitative comparisons across different methods}
    \vspace{-1em}
    \label{fig:rebuttal-baseline-comp}
\end{figure}

% \begin{enumerate}
%     \item \textbf{FID scores of full \& tiny goes up from 50 steps to 16 steps in g=6}
%         \item This table of course conveys various information, but among them, we wanted to say that the training of the model is stable given a certain level of guidance. Please note that the training of the model was recorded as FID 23.97 for the tiny model fixed guidance 8. When the guidance are small, the injection noise are small, and can be close to the guidance = 0 where it’s exactly the same as not having CFG at all. And we know that without CFG image quality is low.
%     \end{enumerate}

% \underline{Reviewer YXGL}
\noindent{\textbf{[\rone] Baselines for other sampling step distillation methods as a comparison for both quantitative and qualitative evaluation:}}
% Most existing distillation methods focus on sampling steps distillation, under the scenario of unguided diffusion models, which make it hard for our CFG distillation method under the guided model setting. That’s why we didn’t include them at the first place. 
% Because most existing distillation methods focus on sampling steps distillation, it is hard for our method to compare with them.
Comparing baselines that only perform sampling step distillation can be hard as they are originally designed under the context of unguided diffusion models, whereas our methods are tailored for guided model.
We included the guided model distillation approach by Meng et al.\footnote{\label{Ondist}  On Distillation of Guided DMs: https://arxiv.org/pdf/2210.03142.pdf}
% and [2]\footnote{\label{Dpm++} DPM++: https://arxiv.org/pdf/2211.01095.pdf} 
in Fig~\ref{fig:rebuttal-baseline-comp} and Tab.~\ref{tab:baselines-compareisons} for comparison.
% We would like to thank the reviewers for this suggestion.
Our method achieves a comparable FID score with the baseline\footref{Ondist} while reducing training computational costs by two orders of magnitude and keeping the original weights in the base model.
% Comparing baselines that only performs sampling step distillation can be difficult because they deal with unguided diffusion models while we methods are used for guided model settings.
% . This poses a challenge for our CFG distillation method when comparing it to existing methods under the guided model setting
% is way lower 
% \item \textbf{Figure 5 is confusing to me. Do the images in one column correspond to the same prompt/starting latent? It is hard for me to judge these images in the way they are presented, am I supposed to compare the 3 teddy bears to the astronaut? And why are the same subjects (chocolate cake, cats) not in the same column?}
% \begin{enumerate}
%     \item reply in combined response, section\textit{ Remaking Fig 5 \& Fig 8. Display Each column with the same textprompts}
% \end{enumerate}
% \item \textbf{Also, is the original guide model the same as the full guide model? If so, why do they have different names in the same figure?}
% \begin{enumerate}
%     \item replied in combined response, section \textit{Original guide model is the Full guide model}
% \end{enumerate}
% \noindent{\textbf{[\rone] Tiny model shown with 50 and 16 steps but the full one with 8 and 16? }}
% The light-weight nature of the tiny model made the performance of 8 steps with varying guidance not as good as full model, and displaying it’s evaluation results may be meaningless. We could add tiny model 8-steps trained on fixed guidance instead.\\
% \noindent{\textbf{[\rone] [{\relax}...]it might be beneficial to include the standard CFG update with x steps in the figure[{\relax}...]}}
% Thanks for reviewers suggestion. We would update \textit{"CFG"} with \textit{"CFG 50 steps"} in Figure 6 accordingly.\\
\input{sec/tab-and-figs/tab-new-comparison}
\noindent{\textbf{[\rone] 
% User study that shows that users do not (strongly) favor Teacher under 50 steps. 
Student images in Fig 6 looks artificial? Conduct a user study that shows that users do not (strongly) favor Teacher under 50 steps:}}
One of the characteristics observed from the injection-based conditioned model (e.g. controlnet) is that the generated images are more saturated and have higher contrast. Some perceive them as less realistic while others may find them more visually pleasing. We conducted a user study where users were presented with a text prompt along with a pair of images generated from that text prompt (Student Full model 50 steps vs Teacher 50 steps) in a sequential fashion. They were asked to choose the preferred image based on image quality and text-image alignment. In the study, 90 participants collectively assessed a total of 680 unique text-image pairs, resulting in the accumulation of 1.8k votes. The vote distribution indicates that users did not strongly favor the teacher, with 1005 votes (55.65 \%) in favor of the teacher and 801 votes (44.35\%) in favor of the student.\\
% The study collected 1.4k votes, revealing that users did not strongly favor the teacher.
% \footnote{680 pairs of unique text-image pairs were collectively evaluated by 45 users. Vote distribution is: Teacher 911(57.62 \%) Student 
%  670(42.38 \%)}. 
% 1005 vs 801
% ADOBE: 8+68 users 822+150(58.34 \%) Student 587+175(41.66 \%)
% This characteristics also persists in our model. But don’t worry, saturation can be alleviate by tuning the guidance number lower.
% We acknowledge that one’s taste over pictures may be more subjective, so we adopt the reviewer’s suggestion to conduct a user study. Specifically, …
% \underline{Reviewer g4Qk}
% \begin{enumerate}
    % \item \textbf{The paper is a bit confusing. For example, it fails to draw a stronger connection to ControlNets, including the crucial detail how the feature maps are "injected" to the main path. I'm assuming this is just an addition like in ControlNet's "zero convolution" paths, but this definitely should be in the text and diagrams to have a self-contained story. Fig 4 is way too abstract}
    % \begin{enumerate}
    %     \item replied in combined response, section \textit{Detailed Tiny model architechture}
    % \end{enumerate}
% \noindent{\textbf{[\rtwo] L337 "In practice" context-setting statements: }}
% We would modify "In practice" to "Without our method" accordingly. We would double-check if there are other similar context-setting that would be confusing to our readers in our camera-ready version.
\noindent{\textbf{[\rtwo] L320 Fixed-guidance discussion}}
    % \begin{enumerate}
        % \item
        Since the tiny guide model only has few trainable parameters, it's challenging for the student to fully mimic the teacher’s output given a \emph{continuous} guidance input. Thus, we also trained a tiny model with fixed guidance. 
        % It would significantly reduce the FID scores from 36.22 to 23.97. 
        The same approach is also used by Meng et al.\footref{Ondist}. \\
    % \end{enumerate}
\noindent{\textbf{[\rtwo] For DDIM, 16 steps is worse than 8 steps in Table 2?
% Also, I don't think these numerical results unambiguously support your story. For example, with g=2,4,6 FID is pretty bad for 50 steps, etc. I'm not satisfied with how the numbers and story combine.
}}
This is a typo - the presented values for 16 steps and 8 steps are reversed. We will revise the table in the camera-ready version.
% \item \textbf{Figures 5 \& 8 [{\relax}...] don't even have fixed prompts per column [{\relax}...] }
% \begin{enumerate}
%     \item reply in combined response, section \textit{Remaking Fig 5 \& Fig 8. Display Each column with the same textprompts}
% \end{enumerate}
% \end{enumerate}
% \underline{Reviewer tesf}

% \begin{enumerate}
%     \item \textbf{I do not understand what the "tiny" guide model architecture is [{\relax}...]}
%     \begin{enumerate}
%         \item replied in combined response, section\textit{ Detailed Tiny model architechture}
%     \end{enumerate}
% \item \textbf{[{\relax}...] I think a much stronger point would be made by using the same text prompts in each column [{\relax}...]}
% \begin{enumerate}
%     \item reply in combined response, section\textit{ Remaking Fig 5 \& Fig 8. Display Each column with the same textprompts}
% \end{enumerate}
\noindent{\textbf{[\rthree] Our methods on pixel-based diffusion models:}}
% Thanks for the reviewer's input. We have been exploring that direction and would include this in our future study.
We thank the reviewer for this interesting avenue for future work, we will add a discussion about applying our method to pixel-based models in the camera-ready version.\\
\noindent{\textbf{[\rone, \rtwo] FID scores of our methods are relatively high when guidance is small (g=2, 4, 6) in Table 2}:}
% Table 2 of course conveys various information, but among them, the main idea we wanted to convey is that the training of the model is stable given a certain level of guidance. Please note that the training of the model was recorded as FID 23.97 for the tiny model fixed guidance 8. When the guidance is small, the injection noise is small, and can be close to the guidance = 0 where it’s the same as not using CFG at all. And we know that without CFG image quality is low.
%We would add this part of the discussion in the original context too.
Table 2 shows that the guide model's performance is stable given a certain level of guidance. Due to the formulation of the guidance model, when the guidance value is small, the injection noise is small (as depicted in Figure 7). Therefore, the g=0 corresponds to not using CFG at all, which is known to generate low-quality images. %This can lead to the decrease in performance as guidance decreases.
However, when guidance is higher (g=8) our model is comparable to the teacher model.\\
\noindent{\textbf{[\rone, \rtwo, \rthree,] Typos, grammatical errors, and context-setting statements:}}
We thank the reviewers for these comments. The manuscript will modified accordingly to avoid confusion in the camera-ready version.


% \color{red}{Tiff TODO:  5. USER study update}\\
% \color{red}{Mentor double-check: 1. Should I include explanation why sampling step distillation will not be provided in our baslines?

% 2. I removed DPM++ currently. Could you help me to double check? 3. I like the idea (probably from Wei-Ann?) of combining lack of baseline sampling step distillation methods + limited tech contribution 4. Should remove apology on L075} 

% \color{red}{TODO: I (@kduarte) have added some comments and optional rewordings (you can search "TODO @ kduarte" in the text.)}

% \end{enumerate}
% \end{enumerate}



==> sec/tab-and-figs/tab-new-comparison.tex <==


\begin{table}[!t]
\centering
\resizebox{0.6\columnwidth}{!}{%
\begin{tabular}{lccc}
\toprule
\textbf{Method}        & \textbf{ODGDM\footref{Ondist} 8 steps}   &     \textbf{Tiny fixed-g 8 steps}  \\ \midrule
% & \textbf{CFG 50 steps (teacher)}                                                      \\ 
FID         &  25-30     
&      \textbf{23.97} 
% & 21 
% Ours-full 8 steps         & 29.53     & \\
% \textbf{Ours-tiny fixed-guidance 8 steps}              & \textbf{23.97}     \\
% Stable Diffusion(Teacher) 50 $\times$ 2 steps            & 21                                        \\ \midrule
% DPM ++\footref{Dpm++} 4 $\times$ 2 steps            & 22.44                     \\ \
% ODGDM\footref{Ondist} 8 steps            & 25-30                                                      \\ \midrule
\end{tabular}
}
\vspace{-1em}
\caption{FID scores comparisons of COCO datasets 30k. Guidance value of our method and the teacher is 8.}
\vspace{-2em}
\label{tab:baselines-compareisons}
\end{table}

% \begin{table}[!t]
% \centering
% \small % or \footnotesize
% \begin{tabular}{@{}ll@{}}
% \toprule
% \textbf{Method}        & \textbf{FID} \\ 
% \midrule
% % Ours-full 8 steps         & 29.53     \\
% \textbf{Ours-tiny fixed-guidance 8 steps}              & \textbf{23.97}     \\
% % Stable Diffusion(Teacher) 50 $\times$ 2 steps            & 21                                        \\
% DPM ++\footref{Dpm++} 4 $\times$ 2 steps            & 22.44                     \\ 
% On Distillation of Guided DM\footref{Ondist} 8 steps            & 25-30                                                      \\ 
% \midrule
% \end{tabular}
% \caption{FID scores comparisons of COCO datasets 30k. Guidance value of our method and the teacher is 8.}
% \label{tab:baselines-comparisons}
% \end{table}
% ```
